Adaptive Geo-Topological Independence Criterion

Testing two potentially multivariate variables for statistical dependence on the basis finite samples is a fundamental statistical challenge. Here we explore a family of tests that adapt to the complexity of the relationship between the variables, promising robust power across scenarios. Building on the distance correlation, we introduce a family of adaptive independence criteria based on nonlinear monotonic transformations of distances. We show that these criteria, like the distance correlation and RKHS-based criteria, provide dependence indicators. We propose a class of adaptive (multi-threshold) test statistics, which form the basis for permutation tests. These tests empirically outperform some of the established tests in average and worst-case statistical sensitivity across a range of univariate and multivariate relationships, offer useful insights to the data and may deserve further exploration.

==> sec_acknowledgements.tex <==
\subsubsection*{Acknowledgements}

The authors would like to thank XXX for their comments on the manuscript. This research was funded by XXX.

==> sec_backup.tex <==

\section{Additional statistical tests}
\label{sec:AKICCD3}

\subsection{Adaptive Gaussian-Kernel Independence Criterion (AKIC)}

AKIC is a kernel-based variant of the ADIC adopting a kernel-based maximized-likelihood approach. Similar to the adaptive searching framework for different thresholds, here the kernel widths were adaptively selected and applied to maximum log likelihood of the dependent association ($H_1$). Given each kernel width, we computed a log likelihood for Gaussian-kernel model using leave-one-out (LOO) cross-validation procedure on the pairwise distance of $X$ and $Y$, and the kernel width with the maximum log likelihood is selected. The logic behind this procedure is that the independence (empirically defined by randomizations) increases the entropy of the joint distribution, therefore, the maximized likelihood of the joint distribution should be higher for the unrandomized distribution given dependence. 
% Figure \ref{fig:AKIC} offers a sketch of this process.


\subsection{Cumulative density difference of distances (CD3)}

The distance-based inflation as an indirect measure of mutual information (introduced in ADIC) can be applied to other properties of the piecewise distance matrix from the multivariate data. We formulate the method as a short-distance inflation (SDI) test: the distribution of distances in the joint space of a dependent association pattern is expected to have a greater prevalence of short distances comparing to the randomized independent pattern, implying a greater concentration of the joint distribution and smaller entropy given any dependence. SDI is computed as the integral of cumulative density within short-distance dominance range: 


\begin{equation}
\label{eq:SDI}
\begin{split}
SDI(X,Y) = & \int_{dom_{start}}^{dom_{end}} [cdfJoint(X-X',Y-Y') \\
& - cdfJoint(X-X',Y_{H_0}-Y'_{H_0})]
\end{split}
\end{equation}
where the $dom_{start}$ and $dom_{end}$ are empirically defined given the probability distribution of the pairwise distances. 
% Figure \ref{fig:CD3} offers a sketch of this process.



\subsection{Asymptotic behaviors for independence}
\label{sec:indeptheory}

This section aims to be prove that the distance correlation computed from GT-transformed distances still satisfies the independence criterion. As the fundamental building blocks of ADIC, distance correlation \cite{szekely2007measuring,szekely2009brownian} generalizes the idea of correlation such that:  
	\begin{itemize}
	\item $\mathcal{R}(X,Y)$ is defined for $X, Y$ in arbitrary dimensions.
    \item $\mathcal{R}(X,Y)=0 \Leftrightarrow X$ and $Y$ are independent.  
	\end{itemize}

Here we wish to extend the proof of these two properties to our adaptive approach, which involves three piecewise functions of linear transformation. For simplicity, we here considered ``GT3'' for our theoretical proof ("GT1'' and ``GT2'' are equivalent linear transformation of ``GT3'' in the region between lower and upper bounds). Consider a \textit{Cauchy sequence} $\{f_n\}^\infty_{n=1}$ in a normed vector space S, it satisfies the existence of an integer for any $\epsilon$ such that, $\norm{f_n - f_m} < \epsilon$ for all $n < N$, $m > N$. The normed vector space $S$ is said to be \textit{complete} if every \textit{Cauchy sequence} converges to a limit in $S$ as a \textit{Banach space}. Here we define $f(X-X')$ as a simplified the geo-topological transformation to be a continuous non-linear \textit{bounded} \textit{functional} onto $L^2[0,1]$:

\begin{equation}
f_n(t) =
  \begin{cases}
0 & \text{if $0 \leq t \leq \frac{1}{2} - \frac{1}{n}$} \\
\frac{1}{2}+ \frac{n}{2}(t-\frac{1}{2}) & \text{if $\frac{1}{2} - \frac{1}{n} \leq t \leq \frac{1}{2} + \frac{1}{n}$} \\
1 & \text{if $\frac{1}{2} + \frac{1}{n} \leq t \leq 1$}
  \end{cases}
\end{equation}

where the upper and lower thresholds defined in section \ref{sec:AGTIC} are replaced with one parameter $n$ (but the theoretical proof is equivalent in the two thresholds case with a linear transformation). From its graph, we see it ``converges'' to:
% a function:

\begin{equation}
\label{eq:functional}
f_0(t) =
  \begin{cases}
0 & \text{if $0 \leq t \leq \frac{1}{2}$} \\
\frac{1}{2} & \text{if $t = \frac{1}{2}$} \\
1 & \text{if $\frac{1}{2} \leq t \leq 1$}
  \end{cases}
\end{equation}

So we can calculate the expected value for the Euclidean distance (within $L^2[0,1]$) after transformation as:

\begin{equation}
\label{eq:EXGT}
\begin{split}
\EX[f(x)] & = \int_0^1 x f(x)dx \\
& = 0+ \int_{\frac{1}{2} - \frac{1}{n}}^{\frac{1}{2} + \frac{1}{n}} x (\frac{nx}{2}+ \frac{1-\frac{n}{2}}{2})dx + \int_{\frac{1}{2} + \frac{1}{n}}^1 x dx \\
% & = \int_{\frac{1}{2} - \frac{1}{n}}^{\frac{1}{2} + \frac{1}{n}} x \frac{nx}{2}dx + \int_{\frac{1}{2} - \frac{1}{n}}^{\frac{1}{2} + \frac{1}{n}}x\frac{1-\frac{n}{2}}{2}dx + \frac{x^2}{2}|_{\frac{1}{2} + \frac{1}{n}}^1 \\
% & = \int_{\frac{1}{2} - \frac{1}{n}}^{\frac{1}{2} + \frac{1}{n}} x \frac{nx}{2}dx + \int_{\frac{1}{2} - \frac{1}{n}}^{\frac{1}{2} + \frac{1}{n}}x\frac{1-\frac{n}{2}}{2}dx + \frac{x^2}{2}|_{\frac{1}{2} + \frac{1}{n}}^1 \\
&=\frac{n}{3x^3}+\frac{n}{4x}-\frac{1}{2n^2}-\frac{1}{4n}+\frac{1}{4}
\end{split}
\end{equation}

which is a monotone nonlinear transformation. In another word, we wish to apply this \textit{monotone nonlinear operator} in a \textit{Hilbert Space} (the original distance correlation). Here we define ${\mathcal{V}^*}^2(X,Y)$ as the dCor calculated given a distance matrix after the proposed geo-topological transformation. If $X$ and $Y$ are independent, then $\EX[XY] = \EX[X]\EX[Y]$

\begin{equation}
\label{eq:dCorGT}
\begin{split}
{\mathcal{V}^*}^2(X,Y) = & \EX[f(\norm{X-X'}_2)f(\norm{f(Y-Y'}_2)] \\
& + \EX [f(\norm{X-X'}_2)] \EX [f(\norm{Y-Y'}_2)] \\
& - \EX [f(\norm{X-X''}_2) f(\norm{Y-Y'}_2) ] \\
& - \EX [f(\norm{X-X'}_2) f(\norm{Y-Y''}_2) ] \\
% = & 2\EX[f(\norm{X-X'}_2) f(\norm{f(Y-Y'}_2)] \\
% & - \EX [f(\norm{X-X''}_2) f(\norm{Y-Y'}_2) ] \\
% & - \EX [f(\norm{X-X'}_2) f(\norm{Y-Y''}_2) ] \\
= & 2\EX[f(\norm{X-X'}_2) f(\norm{f(Y-Y'}_2)] \\
& - 2\EX [f(\norm{X-X'}_2) f(\norm{Y-Y'}_2) ] \\
= & 0 \\
\end{split}
\end{equation}

Thus, the independence criterion still holds regardless of the applied \textit{functional}. Then we are going to look at the threshold searching process to determine whether the independence criterion still holds for ``dCorMax'' (the proof for ``dCorInfMax'' and ``nndCorInfMax'' are theoretically equivalent). We here denote ``dCorMax'' as ${\mathcal{V}^*}^2_{max}(X,Y)$ and define it to be ${\mathcal{V}^*}^2_{max}(X,Y) = \sup_{n\in\mathbb{R}} {\mathcal{V}^*}^2(X,Y)$. 

The equation \ref{eq:functional} is Cauchy, but the convergence is not in the $\sup$ norm: 

\begin{equation}
\label{eq:supConvergence1}
\begin{split}
\norm{f_n-f_0} = & \sup_{t\in[0,1]} |f_n(t)-f_0(t)| = 1/2 \\
\end{split}
\end{equation}

which doesn't converge to zero, but instead, it converges to $f_0$ in the $L^2$ norm as follows:

\begin{equation}
\label{eq:supConvergence2}
\begin{split}
\norm{f_n-f_0}_2 = & \sqrt[]{\int_0^1(f_n(t)-f_0(t))^2dt} \\
%  = & \sqrt[]{\int_{\frac{1}{2}-\frac{1}{n}}^{\frac{1}{2}+\frac{1}{n}}(f_n(t)-f_0(t))^2dt} \\
% \leq & \sqrt[]{\int_{\frac{1}{2}-\frac{1}{n}}^{\frac{1}{2}+\frac{1}{n}}(1)^2dt} \\
% % = & \sqrt[]{(\frac{1}{2}+\frac{1}{n})-(\frac{1}{2}-\frac{1}{n})} \\
% = & \sqrt[]{\frac{2}{n}} \\
\leq & \sqrt[]{\int_{\frac{1}{2}-\frac{1}{n}}^{\frac{1}{2}+\frac{1}{n}}(1)^2dt} = \sqrt[]{\frac{2}{n}} \\
\end{split}
\end{equation}

which converges to zero, showing that the space $L^2[a,b]$ as the completion of all continuous functions (including ``GT'' $f_n(x)$) on $[a,b]$ in the $L^2$ norm. Therefore, ``dCorMax'' still holds the independence criterion. 


==> useful_packages.tex <==
\usepackage{times}
\usepackage{xcolor}
\usepackage{soul}
\usepackage[utf8]{inputenc}
\usepackage[small]{caption}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{caption}
\usepackage{hyperref}

\usepackage{float}
\restylefloat{table}

% the following package is optional:
\usepackage{latexsym} 
\usepackage{booktabs}
\usepackage{amsmath}
\usepackage{verbatim}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{algorithm}
%\usepackage{algorithm2e}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{subfigure}
% \usepackage{natbib}
% \usepackage{booktabs}
% \usepackage{algorithm2e}  %added
% \usepackage{wrapfig}
%\usepackage{breakurl}
%\usepackage[hyphens]{url}
\usepackage{epstopdf}
%\usepackage{endfloat}
\usepackage{lipsum}
\usepackage{color}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

% \usepackage{subcaption}
\usepackage{multicol}

\usepackage{hyperref}
\usepackage{url}

% \def\Rset{\mathbb{R}}
% %\def\C{\mathbb{C}}
% \def\N{\mathbb{N}}
% \def\Z{\mathbb{Z}}
% \def\E{\mathbb{E}}
% \def\P{\mathbb{P}}
% \def\T{\mathcal{T}}
% \def\Var{\mathbb{V}ar}
% \def\rme{\operatorname{e}}
% \newcommand{\1}[1]{\mathbbm{1}_{\left\{#1\right\}}}
% \DeclareMathOperator*{\argmax}{arg\,max}

% \def\ps{P}\def\Ps{\P_\pi}\def\mus{\mu}\def\Es{\E_\pi}
% \def\Xb{\bar{X}}
% \def\F{\mathcal{F}}\def\A{\mathcal{A}}
% \def\eqdef{\triangleq}

